AnyLoc: Towards Universal Visual Place Recognition

Visual Place Recognition (VPR) is vital for robot localization. To date, the most performant VPR approaches are environment- and task-specific: while they exhibit strong performance in structured environments (predominantly urban driving), their performance degrades severely in unstructured environments, rendering most approaches brittle to robust real-world deployment. In this work, we develop a universal solution to VPR -- a technique that works across a broad range of structured and unstructured environments (urban, outdoors, indoors, aerial, underwater, and subterranean environments) without any re-training or fine-tuning. We demonstrate that general-purpose feature representations derived from off-the-shelf self-supervised models with no VPR-specific training are the right substrate upon which to build such a universal VPR solution. Combining these derived features with unsupervised feature aggregation enables our suite of methods, AnyLoc, to achieve up to 4X significantly higher performance than existing approaches. We further obtain a 6% improvement in performance by characterizing the semantic properties of these features, uncovering unique domains which encapsulate datasets from similar environments. Our detailed experiments and analysis lay a foundation for building VPR solutions that may be deployed anywhere, anytime, and across anyview. We encourage the readers to explore our project page and interactive demos: https://anyloc.github.io/.

==> tables/table-main-draft.tex <==

\begin{table*}[!t]
\centering
\caption{Quantitative Results: Performance comparison on six benchmark datasets}
\scalebox{0.95}{
\begin{tabular}{@{}lcccccccccccccc@{}}
\toprule

& \multicolumn{2}{c}{\color{IndoorDark} \indoorChar \hspace{0.1 em} \viewpointChar}  & \multicolumn{2}{c}{\color{IndoorDark} \indoorChar \hspace{0.1 em} \lightingChar} & \multicolumn{2}{c}{\color{IndoorDark} \indoorChar}   & \multicolumn{2}{c}{\color{OutdoorDark} \outdoorChar \hspace{0.1 em} \viewpointChar}   & \multicolumn{2}{c}{\color{OutdoorDark} \outdoorChar}  & \multicolumn{2}{c}{\color{OutdoorDark} \outdoorChar \hspace{0.1 em} \lightingChar}    & \multicolumn{2}{c}{}     \\ 

& \multicolumn{2}{c}{\color{IndoorDark} \textbf{Baidu Mall}}  & \multicolumn{2}{c}{\color{IndoorDark} \textbf{Gardens Point}} & \multicolumn{2}{c}{\color{IndoorDark} \textbf{17 Places}}   & \multicolumn{2}{c}{\color{OutdoorDark} \textbf{Pitts-30k}}   & \multicolumn{2}{c}{\color{OutdoorDark} \textbf{St Lucia}}  & \multicolumn{2}{c}{\color{OutdoorDark} \textbf{Oxford}}    & \multicolumn{2}{c}{\textbf{Average}}     \\ 

\cmidrule(l){2-15} 

\textbf{Methods}                     & R@1            & R@5           & R@1              & R@5           & R@1            & R@5           & R@1            & R@5           & R@1            & R@5         & R@1            & R@5         & R@1            & R@5        \\ 

\cmidrule{1-1} \cmidrule(lr{0.75em}){2-3} \cmidrule(lr{0.75em}){4-5} \cmidrule(lr{0.75em}){6-7} \cmidrule(lr{0.75em}){8-9} \cmidrule(lr{0.75em}){10-11} \cmidrule(lr{0.75em}){12-13} \cmidrule{14-15}

NetVLAD~\cite{arandjelovic2016netvlad}  & 53.05          & 70.55          & 58.50            & 85          & 61.57          & 77.83          & 86.09          & 92.66          & 57.79          & 73.15        & 52.88          & 74.87        & 61.65          & 79.01          \\

CosPlace~\cite{berton2022rethinking} & 41.62          & 55.02          & 74.00            & 94.50          & 61.08          & 76.11          & 90.45          & 95.65          & \textbf{99.79} & 99.93          & 91.10 & 99.47 & 76.34          & 86.78          \\

MixVPR~\cite{ali2023mixvpr}   & 64.44 & 80.28          & 91.50            & 96.00          & 63.79          & 78.82          & \textbf{91.52} & \textbf{95.47} & 99.59          & \textbf{100} & 90.05          & 98.95          & 83.48 & 91.59 \\

CLIP~\cite{radford2021learning}  & 56.02          & 71.60          & 42.50            & 74.50          & 59.36          & 77.59 & 54.97          & 77.20         & 62.70          & 80.67        & 34.55          & 54.97        & 51.69    & 72.75          \\

\dinovtwo{}~\cite{oquab2023dinov2} & 48.95 & 64.44 & 70.50 & 96.00 & 61.58 & 78.82 & 78.26 & 90.96 & 78.21 & 89.55 & 39.79 & 52.88 & 62.88 & 78.78 \\

\rowcolor{Light}
\coolname{} \textit{(DINO L6)}  & 34.69          & 52.75          & 91.50   & 98.00          & 60.34          & 77.34          & 69.82          & 83.17          & 91.67          & 96.93        & 73.30          & 90.58        & 70.22          & 83.13          \\

\rowcolor{Light}
\coolname{} \textit{(DINO L11)} & 63.13          & 79.19 & 88.00            & 98.00   & 64.04 & 79.56          & 82.83          & 91.59          & 84.22          & 93.24        & 28.27          & 53.40        & 68.42          & 82.50          \\

\rowcolor{Light}
\textbf{\coolname{} \textit{(\dinovtwo{})}}   & \textbf{71.03}  & \textbf{84.38} & \textbf{97.50} & \textbf{100} & \textbf{64.29} & \textbf{80.79} & 84.70 & 91.71 & 96.52 & 98.70 & \textbf{91.10} & \textbf{99.48} & \textbf{84.19} & \textbf{92.51}
\\
\bottomrule
\end{tabular}
}
\label{tab:mainResult}
\end{table*}


